MiMo-Audio: Audio Language Models are Few-Shot Learners

Existing audio language models typically rely on task-specific fine-tuning to accomplish particular audio tasks. In contrast, humans are able to generalize to new audio tasks with only a few examples or simple instructions. GPT-3 has shown that scaling next-token prediction pretraining enables strong generalization capabilities in text, and we believe this paradigm is equally applicable to the audio domain. By scaling MiMo-Audio's pretraining data to over one hundred million of hours, we observe the emergence of few-shot learning capabilities across a diverse set of audio tasks. We develop a systematic evaluation of these capabilities and find that MiMo-Audio-7B-Base achieves SOTA performance on both speech intelligence and audio understanding benchmarks among open-source models. Beyond standard metrics, MiMo-Audio-7B-Base generalizes to tasks absent from its training data, such as voice conversion, style transfer, and speech editing. MiMo-Audio-7B-Base also demonstrates powerful speech continuation capabilities, capable of generating highly realistic talk shows, recitations, livestreaming and debates. At the post-training stage, we curate a diverse instruction-tuning corpus and introduce thinking mechanisms into both audio understanding and generation. MiMo-Audio-7B-Instruct achieves open-source SOTA on audio understanding benchmarks (MMSU, MMAU, MMAR, MMAU-Pro), spoken dialogue benchmarks (Big Bench Audio, MultiChallenge Audio) and instruct-TTS evaluations, approaching or surpassing closed-source models. Model checkpoints and full evaluation suite are available at https://github.com/XiaomiMiMo/MiMo-Audio.

==> tables/general_task.tex <==
\begin{table}[htbp]
    \centering
    \small
    \resizebox{0.99\textwidth}{!}{
    % \setlength{\tabcolsep}{4.5pt} % Original comment
    %  current results (s3v7 35kstep) % Original comment
    \begin{tabular}{l c | S[table-format=2.1] S[table-format=2.1] | S[table-format=2.1] S[table-format=2.1] S[table-format=2.1] | S[table-format=2.1] S[table-format=2.1]}
    \toprule
    \multirow{2}{*}{\textbf{Benchmark}}  &  \multirow{2}{*}{\textbf{Metrics}} & \textbf{MiMo-VL} & \textbf{MiMo-VL} & \textbf{Qwen2.5-VL} & \textbf{InternVL3} & \textbf{Gemma-3}  & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{GPT-4o}}} & \multicolumn{1}{c}{{\textbf{Claude 3.7}}} \\
    & & \textbf{7B-SFT} & \textbf{7B-RL} & \textbf{7B} & \textbf{8B} & \textbf{27B-IT} &   & \textbf{Sonnet} \\
    \midrule
    \rowcolor{xiaomiorange!20}
    \multicolumn{9}{l}{\textbf{General}} \\ % Spans 9 columns
    MMMU$_{\mathrm{val}}^{\dag}$          & Acc.         & 64.6  & \textbf{66.7} & 58.6  & 62.7  & 64.9  &   70.7   & 69.8*                \\
    MMMU-Pro$_{\mathrm{standard}}$        & Acc.         & 45.2  & \textbf{46.2} & 34.7* & 45.6* & 37.8* &  42.5*   &  56.5*               \\
    MMMU-Pro$_{\mathrm{vision}}$          & Acc.         & 39.4  & \textbf{40.3} & 29.4* & 37.8* & 24.9* &    36.1*    &  45.8*               \\
    MMBench-en$_{\mathrm{test}}$          &  Acc.        &     \textbf{84.5}  & 84.4 & 83.5  & 83.4  &    81.6*   &    84.6*    &  84.8*               \\
    MMBench-cn$_{\mathrm{test}}$          &  Acc.        &      81.9 & 82.0  & \textbf{83.4} & 82.2  &    82.4*   &    84.5*    &  83.7*               \\
    Mantis                                &  Acc.        & \textbf{78.8} & 78.3  & 74.7* & 72.8* &    70.0*   &  75.6* &  75.1*               \\
    MME-RealWorld$_{\mathrm{en}}$         &  Acc.        & 57.4  & \textbf{59.1} & 57.4  & 56.1* &   51.9*    &    57.5*    &  50.8*               \\
    MME-RealWorld$_{\mathrm{cn}}$         &  Acc.        & 55.0  & 55.5  & 51.2* & \textbf{58.5}* &  47.9*     &    58.5*   &  40.6*               \\
    AI2D                                  &  Acc.        &  83.2 & 83.5 & 83.9  & \textbf{85.2}  & 84.5  &  82.6* &  81.4*               \\ 
    BLINK$_{\mathrm{val}}$                &  Acc.        &  \textbf{62.5} & 62.4 & 56.4  & 55.5  & 53.3* &  60.0  &  62.3*               \\ 
    CV-Bench                              & Acc.         &  81.8 & \textbf{82.3} & 75.4* & 81.0* & 70.4* &  76.0* & 75.4* \\ 
    VibeEval$^{\dag}$                      &  GPT-Score   & 47.2  & \textbf{54.7} & 47.7* & 43.6* & 44.0* & 64.7  &  39.0*               \\ 
    VL-RewardBench$^{\dag}$                &  Macro Acc.  &  61.9 & \textbf{62.7} & 47.3* & 49.7* & 51.9* &  62.4  & 67.4*                \\ 
    V* &  Acc.        &  80.6 & \textbf{81.7} & 73.8* & 72.8* & 50.8* &  73.9  &  {-}               \\  
    VLMs are Blind                        &  Acc.        & 78.0  & \textbf{79.4} & 37.4* & 36.8* &  18.6*     &   49.8*   &  72.1*               \\ 
    PixmoCount                            &  Acc.        &  \textbf{79.4} & \textbf{79.4} & 60.7* & 62.0  &   48.6*    &    54.4*  &  53.5*               \\ 
    CountBench                            &  Acc.        & 87.0  & \textbf{90.4} & 74.1* & 80.0* & 77.2*  &   85.7* &  90.2*               \\ 
    RefCOCO$_{\mathrm{val}}^\mathrm{avg}$              &  Acc.@0.5    & 85.7  & 89.6  & 87.1  & \textbf{90.1} &   {-}    &  {-}      &   {-}              \\  
    \midrule
    \rowcolor{xiaomiorange!20}
    \multicolumn{9}{l}{\textbf{Doc \& OCR}} \\ % Spans 9 columns
    ChartQA$^{\dag}$                      &  Acc.        & \textbf{92.9} & 91.7  & 90.2* & 89.6* & 78.0  &  86.7  & 92.2*                 \\
    CharXiv$_{\mathrm{RQ}}^{\dag}$        &  Acc.        & 54.4  & \textbf{56.5} & 42.5  & 37.6  &  29.2*     &  52.0 &   63.0*              \\
    CharXiv$_{\mathrm{DQ}}^{\dag}$        &  Acc.        &  \textbf{87.0} & 86.8  & 73.9  & 73.6  &   63.8*    &  86.5  &   89.5*              \\
    DocVQA$_{\mathrm{val}}^{\dag}$        &  Acc.        &  95.2 &   \textbf{95.7}    & 95.5* & 89.4* & 86.6  &    93.0*    &   94.1*              \\
    InfoVQA$_{\mathrm{val}}^{\dag}$       &  Acc.        & 87.2  & \textbf{88.0} & 81.4* & 70.7* & 70.6  &  82.1*  &    65.5*             \\
    SEED-Bench-2-Plus                     &  Acc.        & 71.9  & \textbf{72.4} & 70.7  & 69.7  &   66.3*    &   71.1*  & 72.9*                \\
    OCRBench$^{\dag}$                     &  Acc.        & 87.6  & 86.6  & \textbf{89.7}* & 88.0  &   77.6*    & 84.3*  &  80.6*               \\
    \midrule
    \rowcolor{xiaomiorange!20}
    \multicolumn{9}{l}{\textbf{GUI}} \\ % Spans 9 columns
    VisualWebBench$_{\mathrm{avg}}$       &  Acc.        &  \textbf{80.2} & \textbf{80.2}  & 72.9* & 62.7  &    49.7*   & 80.2  &  79.3*               \\
    WebSrc$_{\mathrm{val}}$               &  SQuAD F1    &  \textbf{96.5} & 95.3  & 94.6* & 91.1  &    89.0*   & 89.1*   & 91.1*                \\
    ScreenSpot                            & Center Acc.  &  \textbf{87.3} & 87.2  & 84.7  & 79.5  &   {-}    & 18.3   &  {-}               \\
    ScreenSpot-v2                         & Center Acc.  & 89.5  & \textbf{90.5} & 88.0  & 81.4  &   {-}    & 18.5   &  {-}               \\
    ScreenSpot-Pro$_{\mathrm{avg}}$                & Center Acc.  & 39.9  & \textbf{41.9} & 29.0  &  {-}  &   {-}    & {-}    &   {-}              \\
    OSWorld-G$_{\mathrm{no\_refusal}}$    & Center Acc.  &  54.7 & \textbf{56.1} & 37.5* &  {-}  &   {-}    & {-}    &   {-}              \\
    \midrule
    \rowcolor{xiaomiorange!20}
    \multicolumn{9}{l}{\textbf{Video}} \\ % Spans 9 columns
    Video-MME$_{\mathrm{w/o~sub.}}$                             & Acc.         & 66.9  & \textbf{67.4} & 65.1 & 66.3  &    {-}   & {-}    &     {-}            \\
    Video-MMMU                            & Acc.         &  \textbf{53.1} &   43.3   & 47.4  &   48.9*    &   {-}    & {-}    &    {-}             \\
    EgoSchema$_{\mathrm{val}}$                             & Acc.         & 60.4  & 59.6  & 62.4* &   \textbf{68.2}*   &   {-}   & {-}    &    {-}             \\
    Charades-STA                          & mIoU         &   38.5    & \textbf{50.0} & 43.6  &   25.4    &    {-}   & {-}    &  {-}               \\
    \midrule
    \rowcolor{xiaomiorange!20}
    \multicolumn{9}{l}{\textbf{Text}} \\ % Spans 9 columns
    GPQA Diamond                          & Pass@1       & 56.3 & \textbf{58.3} & 30.3* & 33.5* & 40.9  & 50.6* & 66.0* \\
    SuperGPQA                             & Pass@1       & 42.6 & \textbf{44.3}      & 25.4* & 29.4* & 29.3* & 31.6* & 54.4* \\
    DROP                                  & 3-shot F1    & 82.7 & \textbf{85.1} & 67.6* & 77.5* & 72.2  & 81.5  & 87.2* \\
    MMLU-Pro                              & EM           & 59.8 &  \textbf{64.8}     & 48.7* & 58.3* & 45.3  & 69.1  & 81.0  \\
    IF-Eval                               & Prompt Strict& 75.3 &   75.9    & 75.1* & 87.2* & \textbf{88.9} & 82.5  & 88.7* \\
    \bottomrule
    \end{tabular}
}
    \caption{
        Comparison of \mimovl{} models with other models on diverse visual-language and text benchmarks.
        Results marked with * are obtained using our evaluation framework. $^{\dag}$ indicates that evaluation is performed using GPT-4o. The best results among open-source models are \textbf{bolded}.
    }
    \label{tab:general_updated} % Changed label
\end{table}


% \begin{table}[htbp]
%     \centering
%     \small
%     \resizebox{0.99\textwidth}{!}{
%     % \setlength{\tabcolsep}{4.5pt} % Original comment
%     %  current results (s3v7 35kstep) % Original comment
%     \begin{tabular}{l c | S[table-format=2.1] S[table-format=2.1] | S[table-format=2.1] S[table-format=2.1] S[table-format=2.1] | S[table-format=2.1] S[table-format=2.1]}
%     \toprule
%     \multirow{2}{*}{\textbf{Benchmark}}  &  \multirow{2}{*}{\textbf{Metrics}} & \textbf{MiMo-VL} & \textbf{MiMo-VL} & \textbf{Qwen2.5-VL} & \textbf{InternVL3} & \textbf{Gemma 3}  & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{GPT-4o}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Claude 3.7}}} \\
%     & & \textbf{7B-SFT} & \textbf{7B-RL} & \textbf{7B} & \textbf{8B} & \textbf{12B} &  &  \\
%     \midrule
%     \rowcolor{xiaomiorange!20}
%     \multicolumn{9}{l}{\textbf{General}} \\ % Spans 9 columns
%     AI2D                                  &  Acc.        &  83.2 & 83.5 & 83.9  & \textbf{85.2}  & 84.2  &  82.6* &  81.4*               \\ 
%     BLINK$_{\mathrm{val}}$                &  Acc.        &  \textbf{62.5} & 62.4 & 56.4  & 55.5  & 53.1* &  60.0  &  62.3*               \\ 
%     CV-Bench                              & Acc.         &  81.8 & \textbf{82.3} & 75.4* & 81.0* & 69.3* &  76.0* & 75.4* \\ 
%     MMMU$_{\mathrm{val}}^{\dag}$          & Acc.         & 64.6  & \textbf{66.7} & 58.6  & 62.7  & 59.6  &   70.7   & 69.8*                \\
%     MMMU-Pro$_{\mathrm{standard}}$        & Acc.         & 45.2  & \textbf{46.2} & 34.7* & 45.6* & 33.2* &  42.5*   &  56.5*               \\
%     MMMU-Pro$_{\mathrm{vision}}$          & Acc.         & 39.4  & \textbf{40.3} & 29.4* & 37.8* & 18.2* &    36.1*    &  45.8*               \\
%     MMBench-en$_{\mathrm{test}}$          &  Acc.        &     \textbf{84.5}  & 84.4 & 83.5  & 83.4  &       &    84.6*    &  84.8*               \\
%     MMBench-cn$_{\mathrm{test}}$          &  Acc.        &      81.9 & 82.0  & \textbf{83.4} & 82.2  &       &    84.5*    &  83.7*               \\
%     Mantis                                &  Acc.        & \textbf{78.8} & 78.3  & 74.7* & 72.8* &       &  75.6* &  75.1*               \\
%     MME-RealWorld$_{\mathrm{en}}$         &  Acc.        & 57.4  & \textbf{59.1} & 57.4  & 56.1* &       &    57.5*    &  50.8*               \\
%     MME-RealWorld$_{\mathrm{cn}}$         &  Acc.        & 55.0  & 55.5  & 51.2* & \textbf{58.5}* &       &    58.5*   &  40.6*               \\
%     VibeEval$^{\dag}$                      &  GPT-Score   & 47.2  & \textbf{54.7} & 47.7* & 43.6* & 38.1* & 64.7  &  39.0*               \\ 
%     VL-RewardBench$^{\dag}$                &  Macro Acc.  &  61.9 & \textbf{62.7} & 47.3* & 49.7* & 47.1* &  62.4  & 67.4*                \\ 
%     V* &  Acc.        &  80.6 & \textbf{81.7} & 73.8* & 72.8* & 33.5* &  73.9  &  {-}               \\  
%     VLMs are Blind                        &  Acc.        & 78.0  & \textbf{79.4} & 37.4* & 36.8* &       &   49.8*   &  72.1*               \\ 
%     PixmoCount                            &  Acc.        &  \textbf{79.4} & \textbf{79.4} & 60.7* & 62.0  &       &    54.4*  &  53.5*               \\ 
%     CountBench                            &  Acc.        & 87.0  & \textbf{90.4} & 74.1* & 80.0* & 83.5  &   85.7* &  90.2*               \\ 
%     RefCOCO$_{\mathrm{avg}}$              &  Acc.@0.5    & 85.7  & 89.6  & 87.1  & \textbf{90.1} &       &        &                 \\  
%     \midrule
%     \rowcolor{xiaomiorange!20}
%     \multicolumn{9}{l}{\textbf{Doc \& OCR}} \\ % Spans 9 columns
%     ChartQA$^{\dag}$                      &  Acc.        & \textbf{92.9} & 91.7  & 90.2* & 89.6* & 75.7  &  86.7  &                 \\
%     CharXiv$_{\mathrm{RQ}}^{\dag}$        &  Acc.        & 54.4  & \textbf{56.5} & 42.5  & 37.6  &       &  52.0 &   63.0*              \\
%     CharXiv$_{\mathrm{DQ}}^{\dag}$        &  Acc.        &  \textbf{87.0} & 86.8  & 73.9  & 73.6  &       &  86.5  &   89.5*              \\
%     DocVQA$_{\mathrm{val}}^{\dag}$        &  Acc.        &  95.2 &   \textbf{95.7}    & 95.5* & 89.4* & 87.1  &    93.0*    &   94.1*              \\
%     InfoVQA$_{\mathrm{val}}^{\dag}$       &  Acc.        & 87.2  & \textbf{88.0} & 81.4* & 70.7* & 64.9  &  82.1*  &    65.5*             \\
%     SEED-Bench-2-Plus                     &  Acc.        & 71.9  & \textbf{72.4} & 70.7  & 69.7  &       &   71.1*  & 72.9*                \\
%     OCRBench$^{\dag}$                     &  Acc.        & 87.6  & 86.6  & \textbf{89.7}* & 88.0  &       & 84.3*  &  80.6*               \\
%     \midrule
%     \rowcolor{xiaomiorange!20}
%     \multicolumn{9}{l}{\textbf{GUI}} \\ % Spans 9 columns
%     VisualWebBench$_{\mathrm{avg}}$       &  Acc.        &  \textbf{79.8} & 79.6  & 72.9* & 62.7  &       & 80.2  &  79.3*               \\
%     WebSrc$_{\mathrm{avg}}$               &  SQuAD F1    &  \textbf{96.5} & 95.3  & 94.6* & 91.1  &       & 89.1*   & 91.1*                \\
%     ScreenSpot                            & Center Acc.  &  \textbf{87.3} & 87.2  & 84.7  & 79.5  &       & 18.3   &                 \\
%     ScreenSpot-v2                         & Center Acc.  & 89.5  & \textbf{90.5} & 88.0  & 81.4  &       & 18.5   &                 \\
%     ScreenSpot-Pro$_{avg}$                & Center Acc.  & 39.9  & \textbf{41.9} & 29.0  &  {-}  &       & {-}    &                 \\
%     OSWorld-G$_{\mathrm{no\_refusal}}$    & Center Acc.  &  54.7 & \textbf{56.1} & 37.5* &  {-}  &       & {-}    &                 \\
%     \midrule
%     \rowcolor{xiaomiorange!20}
%     \multicolumn{9}{l}{\textbf{Video}} \\ % Spans 9 columns
%     Video-MME$_{\mathrm{w/o~sub.}}$                             & Acc.         & 66.9  & \textbf{67.4} & 65.1 & 66.3  &    {-}   & {-}    &     {-}            \\
%     Video-MMMU                            & Acc.         &  \textbf{53.1} &   45.4   & 47.4  &   48.9*    &   {-}    & {-}    &    {-}             \\
%     EgoSchema$_{\mathrm{val}}$                             & Acc.         & 60.4  & 59.6  & 62.4* &   \textbf{68.2}*   &   {-}   & {-}    &    {-}             \\
%     Charades-STA                          & mIoU         &   38.5    & \textbf{50.0} & 43.6  &   25.4    &    {-}   & {-}    &  {-}               \\
%     \midrule
%     \rowcolor{xiaomiorange!20}
%     \multicolumn{9}{l}{\textbf{Text}} \\ % Spans 9 columns
%     GPQA Diamond                          & Pass@1       & 56.3 & \textbf{58.3} & 30.3* & 33.5* & 40.9  & 50.6* & 66.0* \\
%     SuperGPQA                             & Pass@1       & 42.6 & \textbf{44.3}      & 25.4* & 29.4* & 29.3* & 31.6* & 54.4* \\
%     DROP                                  & 3-shot F1    & 82.7 & \textbf{85.1} & 67.6* & 77.5* & 72.2  & 81.5  & 87.2* \\
%     MMLU-Pro                              & EM           & 59.8 &  \textbf{64.8}     & 48.7* & 58.3* & 45.3  & 69.1  & 81.0  \\
%     IF-Eval                               & Prompt Strict& 75.3 &   75.9    & 75.1* & 87.2* & \textbf{88.9} & 82.5  & 88.7* \\
%     \bottomrule
%     \end{tabular}
% }
%     \caption{
%         Comparison of \mimovl{} with other models on general visual-language and text benchmarks.
%         Results marked with * are obtained using our evaluation framework. $^{\dag}$ indicates that evaluation is performed using GPT-4o. The best results among open-source models are \textbf{bolded}.
%     }
%     \label{tab:general_updated} % Changed label
% \end{table}


% \begin{table}[htbp]
%     \centering
%     \small
%     \resizebox{0.98\textwidth}{!}{
%     % \setlength{\tabcolsep}{4.5pt} % Original comment
%     %  current results (s3v7 35kstep) % Original comment
%     \begin{tabular}{l c | S[table-format=2.1] | S[table-format=2.1] S[table-format=2.1] S[table-format=2.1] | S[table-format=2.1] S[table-format=2.1]}
%     \toprule
%     \multirow{2}{*}{\textbf{Benchmark}}  &  \multirow{2}{*}{\textbf{Metrics}} & \textbf{\textbf{MiMo-VL}} & \textbf{Qwen2.5-VL} & \textbf{InternVL3} & \textbf{Gemma 3}  & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{GPT-4o}}} & \textbf{Gemini 2.5} \\
%     & & \textbf{7B-RL} & \textbf{7B} & \textbf{8B} & \textbf{12B} &  & \textbf{Flash} \\
%     \midrule
%     \multicolumn{8}{l}{\textbf{General}} \\ % Spans 1 (Benchmark) + 1 (Metrics) + 6 (Models) = 8 columns
%     AI2D                                  &  Acc.        &  83.2 & 83.9  & \textbf{85.2}  & 84.2  &  82.6* &               \\ 
%     BLINK$_{\mathrm{val}}$                 &   Acc.       &  \textbf{62.4} & 56.4  & 55.5  & 53.1* &  60.0  &               \\ 
%     CV-Bench                              & Acc.         &  \textbf{81.8} & 75.4* & 81.0* & 69.3* &  76.0* & 80.1* \\ 
%     MMMU$_{\mathrm{val}}^{\dag}$           & Acc.         & \textbf{66.7}  & 58.6  & 62.7  & 59.6  &        &               \\
%     MMMU-Pro$_{\mathrm{standard}}$        & Acc.         & \textbf{46.2}  & 34.7* & 45.6* & 33.2* &        &               \\
%     MMMU-Pro$_{\mathrm{vision}}$          & Acc.         & \textbf{40.3}  & 29.4* & 37.8* & 18.2* &        &               \\
%     MMBench-en$_{\mathrm{test}}$          &    Acc.      &  \textbf{84.4} & 83.5  & 83.4  &       &        &               \\
%     MMBench-cn$_{\mathrm{test}}$          &    Acc.      &  82.0     & \textbf{83.4}  & 82.2  &       &        &               \\
%     Mantis                                &    Acc.      & \textbf{78.3}  & 74.7* & 72.8* &       &  75.6* &               \\
% % MegaBench & &  &  & &  & &  \\
% MME-RealWorld$_{\mathrm{en}}$         &    Acc.      & \textbf{59.1}  & 57.4  & 56.1* &       &        &               \\
% MME-RealWorld$_{\mathrm{cn}}$         &    Acc.      & 55.5  & 51.2* & \textbf{58.5}* &       &        &               \\
% % mme\_realworld_lite& &  &  & &  & &  \\ 

% % MMstar & &  &  & &  & &  \\ 
% VibeEval$^{\dag}$                     &  GPT-Score   & \textbf{54.7}  & 47.7* & 43.6* & 38.1* & 64.7   &               \\ 
% VL-RewardBench$^{\dag}$               &   Macro Acc. &  \textbf{62.7} & 47.3* & 49.7* & 47.1* &  62.4  &               \\ 
% V* &    Acc.       &  \textbf{81.7} & 73.8* & 72.8* & 33.5* &  73.9  &               \\  
% % VisuLogic                                 &    Acc.      &  23.7 & 26.0  & 28.5* & 25.2* &        &               \\  
% % ZeroBench$_{subq}$  & &  &  & &  & &  \\  
% VLMs are Blind                          &    Acc.      & \textbf{79.4}  & 37.4* & 36.8* &       &        &               \\ 
% PixmoCount                              &    Acc.      &  \textbf{79.4} & 60.7* & 62.0 &       &        &               \\ 
% CountBench                              &    Acc.      & \textbf{90.4}  & 74.1* & 80.0* & 83.5  & 85.7   &               \\ 
% RefCOCO$_{\mathrm{avg}}$               &   Acc.@0.5   & 89.6  & 87.1  & \textbf{90.1}  &       &        &               \\  
% \midrule
% \multicolumn{8}{l}{\textbf{Text-Rich}} \\ % Corrected to span 8 columns
%     ChartQA$^{\dag}$                      &    Acc.      & \textbf{91.7}  & 90.2* & 89.6* & 75.7  & 86.7   &               \\
%     CharXiv$_{\mathrm{RQ}}^{\dag}$        &    Acc.      & \textbf{56.5}  & 42.5  & 37.6  &       & 52.0   &               \\
%     % 
%     CharXiv$_{\mathrm{DQ}}^{\dag}$        &    Acc.      &  \textbf{86.8} & 73.9  & 73.6  &       & 86.5   &               \\
%     DocVQA$_{\mathrm{val}}^{\dag}$        &   Acc.       &    & \textbf{95.5}* & 89.4* & 87.1  &        &               \\
%     InfoVQA$_{\mathrm{val}}^{\dag}$       &   Acc.       & \textbf{88.0}  & 81.4* & 70.7* & 64.9  &        &               \\
%     SEED-Bench-2-Plus                     &    Acc.      & \textbf{72.4}  & 70.7  & 69.7  &       &        &               \\
%     OCRBench$^{\dag}$                     &    Acc.      & 86.6  & \textbf{89.7}* & 88.0  &       & 80.6   &               \\
% \midrule
% \multicolumn{8}{l}{\textbf{GUI}} \\ % Corrected to span 8 columns
% VisualWebBench$_{\mathrm{avg}}$           &    Acc.      &  \textbf{79.6} & 72.9* & 62.7  &       & 78.5   &               \\
%     WebSrc$_{\mathrm{avg}}$               &   SQuAD F1   &  \textbf{95.3} & 94.6* & 91.1  &       & 87.7   &               \\
    
%     ScreenSpot                            & Center Acc.  &  \textbf{87.2} & 84.7  & 79.5  &       & 18.3   &               \\
%     ScreenSpot-v2                         & Center Acc.  & \textbf{90.5}  & 88.0  & 81.4  &       & 18.5   &               \\
%     ScreenSpot-Pro$_{avg}$                & Center Acc.  & \textbf{41.9}  & 29.0  &  {-}  &       & {-}    &               \\
% OSWorld-G$_{\mathrm{no\_refusal}}$    & Center Acc.  &  \textbf{56.1} & 37.5* & {-}   &       & {-}    &               \\
    
% \midrule
% \multicolumn{8}{l}{\textbf{Video }} \\ % Corrected to span 8 columns
%     Video-MME                             & Acc.         & \textbf{67.4}  & 66.6* & 66.3  &       & {-}    &               \\
%     Video-MMMU                            & Acc.         &    & \textbf{47.4}  &       &       & {-}    &               \\
%     EgoSchema                             & Acc.         & 59.6  & \textbf{62.4}* &       &       & {-}    &               \\
%     Charades-STA                          & mIoU         &  \textbf{50.0}   & 43.6  &       &       & {-}    &               \\
% \midrule
% \multicolumn{8}{l}{\textbf{Text}} \\ % Corrected to span 8 columns
%     % CMMLU {\tiny (EM)} & 5-shot & 52.1 & 58.4 & 82.7 &  & & 70.9 \\
%         GPQA Diamond                      & Pass@1       & \textbf{58.3}  & 30.3* & 33.5* &  40.9 & 50.6* & 66.0* \\
%         SuperGPQA                         & Pass@1       &    & 25.4* & 29.4* & 29.3* & 31.6* & 54.4* \\
%         DROP                              & 3-shot F1    & \textbf{85.1} & 67.6* & 77.5* & 72.2  & 81.5  & 87.2* \\
%         MMLU-Pro                          & EM           &    & 48.7* & 58.3* & 45.3  & 69.1  & 81.0   \\
%         IF-Eval                           & Prompt Strict &    & 75.1* & 87.2* & 88.9  & 82.5  & 88.7* \\
%     \bottomrule
%     \end{tabular}
% }
%     \caption{
%         Comparison of \mimovlrl{} with other models on general visual-language benchmarks.
%         Results marked with * are obtained using our evaluation framework. $^{\dag}$ indicates evaluation performed using GPT-4o. The best results among open-source models are \textbf{bolded}.
%     }
%     \label{tab:general} % Suggest changing label if this is a new version
% \end{table}





% \begin{table}[htbp]
%     \centering
%     \small
%     \resizebox{0.98\textwidth}{!}{
%     % \setlength{\tabcolsep}{4.5pt}
%     %  current results (s3v7 35kstep)
%     \begin{tabular}{l c | S[table-format=2.1] S[table-format=2.1] S[table-format=2.1]  | S[table-format=2.1] S[table-format=2.1] |  c}
%     \toprule
%    \multirow{2}{*}{\textbf{Benchmark}}  &  \multirow{2}{*}{\textbf{Metrics}} & \textbf{Qwen2.5-VL} & \textbf{InternVL3} & \textbf{Gemma 3}  & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{GPT-4o}}} & \textbf{Gemini 2.5} & \textbf{\textbf{MiMo-VL}} \\
%    & & \textbf{7B} & \textbf{8B} & \textbf{12B} &  & \textbf{Flash} & \textbf{7B} \\
%     \midrule
%     \multicolumn{8}{l}{\textbf{General}} \\
%     AI2D                           &  Acc.          & 83.9  & 85.2  & 84.2  &  82.6* &       &  83.2 \\ 
%     BLINK$_{\mathrm{val}}$         &   Acc.         & 56.4  & 55.5  & 53.1* &  60.0  &       &  62.5\\ 
%     CV-Bench                       & Acc.           & 75.4* & 81.0* & 69.3* &  76.0* & 80.1* &  81.8\\ 
%     MMMU$_{\mathrm{val}}^{\dag}$   & Acc.           & 58.6  & 62.7  & 59.6  &        &       & 64.6 \\
%     MMMU-Pro$_{\mathrm{standard}}$ & Acc.           & 34.7* &     45.6*  & 33.2* &        &       & 45.2
%   \\
%     MMMU-Pro$_{\mathrm{vision}}$   & Acc.           & 29.4* &     37.8*  & 18.2* &        &       & 39.4 \\
%     MMBench-en$_{\mathrm{test}}$   &     Acc.       & 83.5  & 83.4  &       &        &       &  \\
%     MMBench-cn$_{\mathrm{test}}$   &      Acc.      & 83.4  & 82.2  &       &        &       &  \\
%     Mantis                         &        Acc.    & 74.7* & 72.8* &       &  75.6* &       & 78.8  \\
% % MegaBench & &  &  & &  & &  \\
% MME-RealWorld$_{\mathrm{en}}$      &      Acc.      & 57.4  & 56.1* &       &        &       & 57.4 \\
% MME-RealWorld$_{\mathrm{cn}}$      &      Acc.      & 51.2* & 58.5* &       &        &       & 55.0 \\
% % mme\_realworld_lite& &  &  & &  & &  \\ 

% % MMstar & &  &  & &  & &  \\ 
% VibeEval$^{\dag}$                  &  GPT-Score     & 47.7* & 43.6* & 38.1* & 64.7   &       & 47.2

%  \\ 
% VL-RewardBench$^{\dag}$            &   Macro Acc.   & 47.3* & 49.7* & 47.1* &  62.4  &       &  61.9\\ 
% V*                                 &     Acc.       & 73.8* & 72.8* & 33.5* &  73.9  &       &  80.6\\  
% % VisuLogic                          &       Acc.     & 26.0  & 28.5* & 25.2* &        &       &  23.7\\  
% % ZeroBench$_{subq}$  & &  &  & &  & &  \\  
% VLMs are Blind                     &      Acc.      & 32.9* & 35.8* &       &        &       &  78.0\\ 
% PixmoCount                         &     Acc.       & 60.7* &      62 .0 &      &        &       &  79.4
% \\ 
% CountBench                         &        Acc.    & 74.1* & 80.0* & 83.5  & 85.7   &       & 87.0 \\ 
% RefCOCO$_{\mathrm{avg}}$           &     Acc.@0.5   & 87.1  & 90.1  &       &        &       & 85.7 \\  
% \midrule
% \multicolumn{8}{l}{\textbf{Text-Rich}} \\
%    ChartQA$^{\dag}$                         &      Acc.      & 90.2* & 89.6* & 75.7  & 86.7   &       & 92.9  \\
%    CharXiv$_{\mathrm{RQ}}^{\dag}$  &       Acc.     & 42.5  & 37.6  &       & 52.0   &       & 54.4 \\
%    % 
%    CharXiv$_{\mathrm{DQ}}^{\dag}$  &      Acc.      & 73.9  & 73.6  &       & 86.5   &       &  87.0 \\
%     DocVQA$_{\mathrm{val}}^{\dag}$        &    Acc.        & 95.5* & 89.4* & 87.1  &        &       & 95.2  \\
%    InfoVQA$_{\mathrm{val}}^{\dag}$        &    Acc.        & 81.4* & 70.7* & 64.9  &        &       & 87.2 \\
% SEED-Bench-2-Plus                  &       Acc.     & 70.7  & 69.7  &       &        &       & 71.9  \\
%    OCRBench$^{\dag}$                        &       Acc.     & 89.7* & 88.0  &       & 80.6   &       & 87.6 \\
% \midrule
% \multicolumn{6}{l}{\textbf{GUI}} \\
% VisualWebBench$_{\mathrm{avg}}$    &      Acc.      & 72.9* & 62.7  &       & 78.5   &       &  79.8 \\
%    WebSrc$_{\mathrm{avg}}$         &   SQuAD F1     & 94.6* & 91.1  &       & 87.7   &       &  96.5 \\
   
%    ScreenSpot                      & Center Acc.    & 84.7  & 79.5  &       & 18.3   &       &  87.3\\
%    ScreenSpot-v2                   & Center Acc.    & 88.0  & 81.4  &       & 18.5   &       & 89.5 \\
%    ScreenSpot-Pro                  & Center Acc.    & 29.0  &       &       & {-}    &       & 39.9 \\
% OSWorld-G$_{\mathrm{no\_refusal}}$ & Center Acc.    & 37.5* &       &       & {-}    &       &  54.7\\
   
% \midrule
% \multicolumn{6}{l}{\textbf{Video }} \\
%    Video-MME                       & Acc.           & 66.6* & 66.3  &       & {-}    &       & 66.9 \\
%    Video-MMMU                      & Acc.           & 47.4  &       &       & {-}    &       & 53.1 \\
%    EgoSchema                       & Acc.           & 62.4* &       &       & {-}    &       & 60.4 \\
%    Charades-STA                    & mIoU           & 43.6  &       &       & {-}    &       &  \\
% \midrule
% \multicolumn{6}{l}{\textbf{Text}} \\
%     % CMMLU {\tiny (EM)} & 5-shot & 52.1 & 58.4 & 82.7 &  & & 70.9 \\
%         GPQA Diamond               & Pass@1         & 30.3* & 33.5* &  40.9 & 50.6* & 66.0*  & 58.0*\\
%         SuperGPQA                  & Pass@1         & 25.4* & 29.4* & 29.3* & 31.6* & 54.4*  & 42.8* \\
%         DROP                       & 3-shot F1      & 67.6* & 77.5* & 72.2  & 81.5  & 87.2*  & 82.7* \\
%         MMLU-Pro                   & EM             & 48.7* & 58.3* & 45.3  & 69.1  & 81.0   & 59.8* \\
%         IF-Eval                    & Prompt Strict  & 75.1* & 87.2* & 88.9  & 82.5  & 88.7*  & 66.3*\\
%     \bottomrule
%     \end{tabular}
% }
%     \caption{
%         Comparison of \mimovl{} with other models on general visual-language benchmarks.
%         Results marked with * are obtained using our evaluation framework. $^{\dag}$ indicates evaluation performed using GPT-4o.
%     }
%     \label{tab:base_eval}
% \end{table}








